Frame-Semantic Parsing with Softmax-Margin Segmental RNNs and a Syntactic Scaffold

We present a new, efficient frame-semantic parser that labels semantic arguments to FrameNet predicates. Built using an extension to the segmental RNN that emphasizes recall, our basic system achieves competitive performance without any calls to a syntactic parser. We then introduce a method that uses phrase-syntactic annotations from the Penn Treebank during training only, through a multitask objective; no parsing is required at training or test time. This "syntactic scaffold" offers a cheaper alternative to traditional syntactic pipelining, and achieves state-of-the-art performance.

==> data.tex <==
\section{Detailed Data and Task}
\label{sec:data}

\todo{shorten and move to experiments section.}
We use two linguistic resources which we describe below, FrameNet
\citep{Baker:98} and the Penn Treebank~\citep{Marcus:93}.
We also use GloVe~\citep{Pennington:14} pre-trained word embeddings of size 100,
trained on a corpus of 6 billion words.\ark{Don't know if this is necessary in
this section... I'd put it in the pre-processing part, not as your "main" training dataset.}

\subsubsection{FrameNet}

The FrameNet lexicon contains an ontology of manually
identified semantic frames, a corpus of \term{full-text} annotated
sentences, and a corpus of partially annotated \term{exemplar} annotated
sentence.
A frame is a generic event, situation, or relationship\sam{is this
list exhaustive?} that has a set of semantic roles (frame elements) associated
with it, and a set of lexical units that have been seen to evoke it in corpus study.
In frame-semantic theory, when a lexical unit is read or heard in a sentence,
the frame and its frame elements are brought to mind whether or not they are explicitly
mentioned.
To compare to related work we use FrameNet release 1.5, but we also
report our results on the latest release at the time of writing, FrameNet 1.7
(available at \url{http://framenet.icsi.berkeley.edu}).

\sam{
FN stats:
How many frames, frame elements?
Avg size of $|\rolesForF|$?
}

\paragraph{Exemplars}
Each lexical unit has a set of exemplar annotations.
FrameNet lexicographers searched for the lexical unit in a corpus, and chose
exemplars in order to illustrate and cover the full range of syntactic variations possible.
Exemplar sentences make up the bulk of FrameNet's annotations (XXXk sentences
in FrameNet 1.7), but are annotated for a single frame only, and because of the
search-based annotation procedure they can't be thought of as samples from
any natural distribution.

\paragraph{Full-text}
FrameNet's full-text annotations are fewer (Xk sentences), but have
been found to be more useful for training automatic frame-semantic parsing
systems~\cite{Das:14}.
In the full-text corpus, documents were annotated sentence by sentence, with an
attempt made to identify and annotate every frame and its arguments.

\sam{
Corpus stats:
How many sentences (1.5 vs 1.7)?
What domain is the full-text?
How many targets per sentence?
How many arguments per frame?
What percent of targets are N, V, JJ, etc.?
}




% \paragraph{Penn TreeBank}

% Relative to PropBank~\cite{Palmer:05}, FrameNet has a larger label set and a
% smaller full-text corpus, which makes automatic parsing difficult and limits the complexity of
% models that can be learned.

% Its argument spans roughly correspond to syntactic constituents, but not
% exactly.

\subsection{Frame-Semantic Parsing}
\label{sect:task}

We follow \citet{Das:14} in modeling frame-semantic parsing as a pipeline of
target identification, frame identification, and then argument
identification.

\paragraph{Target Identification (\term{target id})}
The first subtask in the frame-semantic parsing pipeline is to identify
the \term{targets} in a sentence, the words and phrases that evoke frames.
For example in \figu{fig:dryingup}, \textit{``played''}, \textit{``major''},
\textit{``preventing''}, and \textit{``drying up''} are targets.
We follow prior work and use gold targets in our experiments.

\paragraph{Frame Identification (\term{frame id})}
For each identified target, we must identify which frame it evokes.
In \figu{fig:dryingup},
\textit{``played''} evokes the \fnframe{Performers\_and\_roles} frame,
\textit{``major''} evokes the \fnframe{Importance} frame,
\textit{``preventing''} evokes the \fnframe{Thwarting} frame,
and \textit{``drying up''} evokes the \fnframe{Becoming\_dry} frame.
Although we do address frame identification,
% so that we have a full frame-semantic parsing system
our frame id model is a natural and uninteresting simplification of our arg id
model, so we relegate its details to Appendix~\ref{sect:frameid}.


\paragraph{Argument Identification (\term{arg id})}
The final subtask of frame-semantic parsing is to identify and label
the arguments of each frame.
For each frame $f$, FrameNet defines a set $\rolesForF$ of \term{frame elements},
which are semantic roles specific to that frame.
Whenever a frame $f$ is evoked in a sentence $\seq{x}$, each of its frame
elements $y \in \rolesForF$ is realized in the sentence as a set of tokens, called an
\term{argument}.
In general, arguments are either a contiguous span, $\seq{x}_{i:j}$, or the
empty set, $\emptyset$ (in which case it is called a \term{null instantiation}).
For example, in the \fnframe{Importance} frame in \figu{fig:dryingup}, the
span \textit{``role''} fills the \fnrole{Factor} role, \textit{``in
preventing Las Vegas from drying up''} fills the \fnrole{Undertaking} role, and
the \fnrole{Interested\_party} role is null-instantiated
(\fnframe{Importance} has additional roles that are also null-instantiated and
not pictured in \figu{fig:dryingup}).
In rare cases, an argument can be a set of two spans.
Two arguments of the same frame must not overlap.\footnote{
Arguments are known to follow other constraints as well, such as mutual
exclusion or requirement between specific roles, and contiguousness.
\citet{Tackstrom:15} gives a dynamic program to enforce all of the constraints,
but it has runtime that is exponential in the number of roles.
Beam-search and AD$^3$ have been succesfully used \sam{cite DDas, Martins},
but also slow down inference.
In this work, we opt for simpler semi-Markov inference at the expense
of possibly violating unenforced constraints.}
% \begin{itemize}
%   \item two arguments of the same frame must not overlap,
%   \item certain roles are mutually exclusive \sam{give ex?},
%   \item certain roles, if instantiated, require another certain role to be
%   instantiated \sam{give ex?}, and
%   \item (optionally) an argument consists of at most one contiguous span. 
% \end{itemize}
Argument identification is a special case of PropBank-style
span-based semantic role labeling~\cite{Carreras:05}\sam{not really. needs
clarification.}.
Argument identification is the most challenging subtask of frame-semantic
parsing and is the primary focus of this work~\sect{sect:argid}.

